PERMUTATION Strikes Back: The Power of Recourse in Online Metric Matching

In the classical Online Metric Matching problem, we are given a metric space with $k$ servers. A collection of clients arrive in an online fashion, and upon arrival, a client should irrevocably be matched to an as-yet-unmatched server. The goal is to find an online matching which minimizes the total cost, i.e., the sum of distances between each client and the server it is matched to. We know deterministic algorithms~\cite{KP93,khuller1994line} that achieve a competitive ratio of $2k-1$, and this bound is tight for deterministic algorithms. The problem has also long been considered in specialized metrics such as the line metric or metrics of bounded doubling dimension, with the current best result on a line metric being a deterministic $O(\log k)$ competitive algorithm~\cite{raghvendra2018optimal}. Obtaining (or refuting) $O(\log k)$-competitive algorithms in general metrics and constant-competitive algorithms on the line metric have been long-standing open questions in this area. In this paper, we investigate the robustness of these lower bounds by considering the Online Metric Matching with Recourse problem where we are allowed to change a small number of previous assignments upon arrival of a new client. Indeed, we show that a small logarithmic amount of recourse can significantly improve the quality of matchings we can maintain. For general metrics, we show a simple \emph{deterministic} $O(\log k)$-competitive algorithm with $O(\log k)$-amortized recourse, an exponential improvement over the $2k-1$ lower bound when no recourse is allowed. We next consider the line metric, and present a deterministic algorithm which is $3$-competitive and has $O(\log k)$-recourse, again a substantial improvement over the best known $O(\log k)$-competitive algorithm when no recourse is allowed.

==> app-line.tex <==
\section{Proofs for \Cref{sec:line} (Matching on Line metric)} \label{app:line}


\begin{proofof}{\Cref{lem:no-middle-server}}
    We will first prove that if we execute \permutation algorithm on line, there are no free servers inside any arc. 
    Recall that \permutation maintains an offline optimal matching $\mathcal{M}_t^*$ at time $t$, and when a client $c_t$ arrives, we pair it with the server that is present in $\mathcal{M}_t^* \setminus \mathcal{M}_{t-1}^*$. 
    In fact, the symmetric difference of $\mathcal{M}_t^*$ and $\mathcal{M}_{t-1}^*$ is an augmenting path starting at $c_t$ and ending at $s_t$. 
    Let it be denoted by $c_t,s_{p_1},c_{p_1},\ldots,s_{p_m}=s_t$. The edges $(c_t,s_{p_1}),(c_{p_1},s_{p_2}),\ldots$ are the new edges, and the rest $(s_{p_1},c_{p_1}),(s_{p_2},c_{p_2}),\ldots$ are the old edges. 
    Recall that the cost of $\mathcal{M}_{t}^*$ is at least that of $\mathcal{M}_{t-1}^*$, and thus, in the augmenting path, the cost of new edges is at least that of the old edges.
    
    We claim a stronger property that in any suffix of the augmenting path, the cost of the new edges is at least that of old edges. 
    Consider a suffix $s_{p_i},c_{p_i},\ldots,s_{p_m}$. 
    If the cost of new edges is less than the old edges, we can change the old matching from $(s_{p_i},c_{p_i}),\ldots,s_{p_{m-1}},c_{p_{m-1}})$ to $(c_{p_i},s_{p_i}),\ldots,(c_{p_m},s_{p_m})$ while keeping the rest of the edges intact to get a matching with cost less than $\mathcal{M}_{t-1}^*$, contradicting the fact that $\mathcal{M}_{t-1}^*$ is an optimal matching for the first $t-1$ clients. 
    Now, suppose that there is a free server $s*$ in between $c_t$ and $s_t$. 
    Consider the suffix of the augmenting path ending at $s'$. 
    Let $\mathcal{M}'_{t}$ be the matching obtained from $\mathcal{M}_{t-1}^*$ by adding the new augmenting path ending at $s'$. 
    Since the cost of new edges is at least that of old edges in any suffix of the original augmenting path, the cost of the new augmenting path (in terms of the difference between new and old edges) is at most that of the old augmenting path. 
    And thus, the cost of the matching $\mathcal{M}'_t$ is at most that of $\mathcal{M}_{t}^*$. 
    Furthermore, if we assume that the location of all the clients and servers are distinct, the cost of $\mathcal{M}'_t$ is in fact strictly smaller than $\mathcal{M}_{t}^*$, contradicting the fact that $\mathcal{M}_{t}^*$ is an optimal matching of first $t$ clients. 
    This proves the claim that when we execute \permutation on the line metric, there are no free servers inside any arc.
    
    Using this, we will prove using induction on $t$ that after the arrival of $t$ clients, there are no free servers inside any arcs when executing \recursivecancel. 
    At $t=1$, we are adding an edge directly from \permutation, hence the claim follows trivially. 
    Consider the scenario when we are adding a client server pair $(c_t,s_t)$. 
    If the edge $(c_t,s_t)$ is a forward arc, we add it directly, and all other matches are unaffected. 
    As $(c_t,s_t)$ is added directly from \permutation, there are no free servers inside it, and thus proving the inductive claim. 
    Consider the case when $(c_t,s_t)$ is a backward arc. 
    As this edge is given by \permutation, there are no free servers inside the backward arc.
    This combined with the fact that the cancellation of the algorithm only adds segments inside $[\ell(s_t),\ell(c_t)]$ to arcs ensures that all the new arcs formed during recursive addition of $(c_t,s_t)$ don't contain any free servers. 
    
\end{proofof}

\begin{proofof}{\Cref{lem:shrink}}
	Note that once a server is matched by a backward arc, it is not going to change its match from that point onward. Hence, we can assume that $c_1$ to $s$ is a forward arc. 
	Also note that in a single iteration of the algorithm, each server is rematched at most once in the recursive step. 
	
	Consider the iteration of ~\Cref{alg:recursivecancel} in which we rematch server $s$ from $c_1$ to $c_2$.  
	Let $(s',c')$ be the backward arc that was obtained from \permutation. During the recursive step of the iteration, $c_1,s$ intersected with backward arc $c_2,s'$, and thus the match of $s$ is changed from $c_1$ to $c_2$.
	This implies that $c_2$ is to the right of $c_1$ since otherwise, the two arcs would not have intersected in the first place.
\end{proofof}

\begin{proofof}{\Cref{lem:suffix}}
	Let $A$ denote the set of clients and servers prior to adding $c$ and $s$. Let $x \in [\ell(c),\ell(s)]$. We are interested in the suffix $[x,\ell(s)]$ of the arc $c,s$. Introduce a virtual client $c'$ at $x$. Consider the optimal solution of $A \cup \{c',s\}$. 
	%Since we are following Permutation till before $c$ is added, the optimal cost of matching $A \cup \{c',s\}$ is at least the optimal cost of matching $A$.
	We claim that the optimal cost of matching $A \cup \{c',s\}$ is at least the optimal cost of matching $A$.
	Note that if we add $c'$ to $A$, \permutation might not choose to pair it with $s$. However, irrespective of which client-server pair we add, the optimal solution can only go up. If not, we can take a subset of the new matching ignoring the new client and get a solution of lower cost to the previous instance. 
	Thus, obtaining a contradiction to the fact that \permutation maintains a solution that is server-optimal.
	
	When we add $\{c',s\}$ to $A$, the increase in the cost of optimal matching occurs precisely at the intervals where the number of clients to the left is greater than the number of servers (after adding $c',s$). And in other intervals in $[x,\ell(s)]$, the cost paid by the optimal matching decreases. 
	However, this exactly corresponds to the redundancy and non-redundancy of the forward arc $c,s$ within intervals inside $[x,\ell(s)]$. The intervals where the cost of optimal matching increases are the ones which are non-redundant, and the intervals where the cost of optimal matching decreases are the ones which are redundant. 
\end{proofof}

\begin{proofof}{\Cref{lem:redundant}}
	In fact,  we prove a stronger claim inductively on the number of client-server pairs added:
	\begin{enumerate}
		\item In any interval, the number of redundant forward arcs is equal to the minimum of the number of forward and the number of backward arcs crossing this interval. 
		\item In any interval, if both redundant and non-redundant forward arcs are present, then the server of the non-redundant arc is to the right of the server of redundant arc. 
	\end{enumerate}
	Let $c,s$ be the client-server pair given by \permutation.
	Consider the two cases, adding a forward arc and a backward arc. 
	\begin{enumerate}
		\item Suppose that $s$ is to the right of $c$ i.e. the case when we add the forward arc directly. 
		If in an interval between $c$ and $s$, there are fewer forward arcs than backward arcs prior to adding $c$ and $s$, we mark that interval as a redundant interval. Observe that this ensures that in those intervals, redundant forward arc count increases, and is equal to the minimum of the number of forward and the number of backward arcs crossing the interval. 
		In intervals where the number of forward arcs is at least the number of backward arcs prior to adding $c$ and $s$, the interval is non-redundant. In this case, the minimum of forward and backward arcs does not increase, and thus this ensures that the claim continues to remain valid. 
		
		For the second claim: If in an interval, the new arc is marked redundant, then all the forward arcs in that interval are redundant. If in an interval, the new arc is marked non-redundant, we need to show that the new server is to the right of any server whose arc is marked redundant. This follows directly from the fact that an unmatched server cannot be present in the middle of an arc (by optimality of the \permutation algorithm), and hence, $s$ is to the right of the server of any forward arc that intersects $c,s$. 
		
		\item Suppose that $s$ is to the left of $c$ i.e. the case when we recursively add backward arc(s). 
		From Lemma~\ref{lem:shrink}, we know that the forward arcs corresponding to a server only shorten. Thus, the second claim trivially follows. 
		
		The algorithm deletes a forward arc from the intervals between $s$ and $c$ where there is at least one forward arc. 
		If the number of forward arcs in an interval is at most the number of backward arcs, then all of them are redundant arcs, and we delete one redundant one. The property of claim $1$ still holds. 
		Thus, it remains to show that if there are both non-redundant and redundant arcs in an interval, our algorithm deletes the non-redundant one. 
		We use claim $2$ here. If there are both redundant and non-redundant arcs in an interval, note that the server corresponding to the non-redundant arc is to the right of the server corresponding to the redundant arc. 
		
		Recall that there is at most one forward arc that is deleted from any interval. 
		If a redundant arc is deleted from an interval, when the arc is selected, it has the farthest server among all arcs that intersect the backward arc. This combined with the above fact implies that if a redundant arc is deleted from an interval, then there is no non-redundant arc in that interval. Thus, if there are both redundant and non-redundant forward arcs inside an interval, our algorithm deletes the non-redundant arc. 
	\end{enumerate}
\end{proofof}

\begin{proofof}{\Cref{lem:shorten}}
	Suppose for the sake of contradiction that $s'$ is to the right of $s$. 
	Note that once a client gets matched via a backward arc, the algorithm does not rematch it. 
	Thus, $c$ is to the left of $s$, and thus to the left of $s'$. 
	As $c$ is in the list of clients when the algorithm considers $s'$, it is in the list when the algorithm considers $s$ as well. Thus, $s$ should not have been rematched. 
\end{proofof}

\begin{proofof}{\Cref{lem:unique-server}}
	Fix the iteration as adding a backward arc $c,s$. We will prove the Lemma by inducting on the number of vertices (union of clients and servers) visited by the algorithm in the iteration. 
	Let $c'$ be the client matched with $s$ by the algorithm. 
	Note that $c'$ is the second vertex visited by the algorithm. 
	At this point, the server $s'$ that is originally matched to $c'$ is the only server satisfying the above property. 
	This covers the base case of the induction. 
	
	Suppose that the property is true till we add a new vertex $p$. 
	If $p$ is a client, adding $p$ to the list or matching it with a server to the left of it does not rematch any clients of servers yet unconsidered by the algorithm. 
	If $p$ is a server, if it is the unique server whose client has already been rematched, we now get a new server added to $list$. 
	If it has not lost its client yet, the set of servers whose clients are lost does not change (by design of the algorithm). 
\end{proofof}
    


==> fully-online.tex <==
\section{Dynamic Online Matching}
\label{sec:general-metrics}

In this section, we look at the dynamic version of the problem: at the beginning of the instance, a set of servers $S_0$ is available for matching. At $t$: one of four possible events can happen, {\it (i) client arrival:} a new client request $c_t$ arrives and must be matched to some server;  {\it (ii) server departure:} an existing server departs, potentially requiring the client it was matched with to be rematched; {\it (iii) server arrival:} a new server arrives; and {\it (iv) client departure:} an existing client departs. In all cases, the algorithm is allowed to re-match existing clients, incurring a recourse equal to the number of re-matches.

In comparison to previous sections, we no longer have the nested set of clients and servers since there are departures. However, for sake of clarity in presentation, we abuse notation and let the set of clients present in the system at time $t$ be denoted by $C_t$, and the set of servers present in the system at time $t$ by $\Scal_t$ the online matching by $M_t$, and the optimal offline matching of clients $C_t$ by $\Mcal_t$. For feasibility, we assume that $|S_t| \geq |C_t|$ for all $t$. Unlike in the previous case where only client arrivals necessitate changes to existing matching, in the dynamic case, any of the four types of events can do so. 

To give the algorithm for a general metric, we begin by giving an algorithm for a special class of Tree metric called Hierarchically Well-Separated Trees (HST), and then invoking a classical result of \cite{fakcharoenphol2004tight} on low-distortion embedding of general metrics into tree metrics.

We borrow the following background on HST's and tree embeddings from \citep{bansal2007log}. 

\begin{definition}[Hierarchically Well-Separated Trees] An  $\alpha$-Hierarchically Well-Separated Tree for a given parameter $\alpha > 1$ is a rooted tree $T=(V,E)$ along with a length function $c()$ on the edges which satisfies the following properties:
\begin{enumerate}
    \item For each node $v$, all its children are at the same distance from $v$.
    \item For any node $v$, $c(p(v), v) \geq \alpha c(v, c(v))$ where $p(v)$ is parent of $v$ and $c(v)$ is any child of $v$. That is, the length of the edges increase geometrically going from leaves to the root.
    \item Each leaf has the same distance to its parent.
\end{enumerate}
\end{definition}

Therefore, we can view an $\alpha$-HST as a tree with depth $D$: the root is at {\it level} $D$, and all the leaves are at level $1$. For a leaf $x$ matched to a leaf $y$ (one a client, and the other corresponding to a server)  the {\it level} of the match is defined as the level of the lowest common ancestor of $x$ and $y$ in the tree. The following theorem shows that any general metric can be embedded into a distribution of HST's.

\begin{theorem}[\citep{fakcharoenphol2004tight}] 
Given any metric $(\Xcal, d)$ on $k$ points, there is a probability distribution on $\alpha$-HST's (Hierarchically Well Separated) such that: {\it (i)} For each tree $T$ in the support of the distribution, the leaves of $T$ correspond to the nodes of $\Xcal$, {\it (ii)} the tree distance is at least the metric distance: $d_T(x,y) \geq d(x,y)$ for all $x,y \in \Xcal$, and {\it (iii)} The expected tree distance satisfies: $\expct{d_T(x,y)} \leq \Ocal(\alpha \log k) d(x,y)$ for all $x,y \in \Xcal$.
\end{theorem}

A choice of $\alpha=2$ will suffice for us. \citet{fakcharoenphol2004tight}, also prove that the distribution can be efficiently sampled from, and further that the height $D$ of the $\alpha$-HST is bounded by $\Ocal(\log \Delta)$ with probability 1. In summary, for any $k$-point general metric with aspect ratio $\Delta$, there exists a distribution of trees with depth at most $\Ocal(\log \Delta)$ such that all distances are preserved within a factor of  $\Ocal(\log k)$. 

Next we give our main result for dynamic online min-cost matching on a tree metric. We defer the proof to Section~\ref{sec:dynamic_HST} where we describe the algorithm and analyze its performance. 

\begin{theorem}
\label{thm:dynamic_HST}
There exists a $(1, D)$-competitive deterministic algorithm for online min-cost matching on an HST of depth $D$.
\end{theorem}

That is, for an HST, the matching maintained by the algorithm is in fact optimal. Further, the number of recourse steps is at most $D$ per arrival/departure event (and not just on average).

\begin{corollary}
\label{cor:dynamic_HST}
For any $k$ point metric with aspect ratio $\Delta$, there exists a randomized online algorithm which is $( \Ocal(\log k),  \Ocal(\log \Delta))$-competitive for min-cost matching against an oblivious adversary.
\end{corollary}
\begin{proof}
The algorithm proceeds by first sampling a $2$-HST given the $k$-point metric, and then executes the Algorithm from Theorem~\ref{thm:dynamic_HST}. Since the depth of the tree is $\Ocal(\log \Delta)$ with probability 1, this implies the recourse bound in the corollary. 

To bound the cost, let $T$ denote the tree sampled during the construction of the $2$-HST, and let $M_t$ denote the matching produced by the algorithm (which is also a random quantity). Recall that we denote the optimal matching at time $t$ by $\Mcal_t$. Let the cost of a matching $M$ under the metric induced by tree $T$ be denoted by $\cost_T$.

By the optimality of the matching produced for the particular tree sampled, we get:
\begin{align*}
    \cost_T(M_t) & \leq \cost_T(\Mcal_t),
\end{align*}
which combined with the second property gives:
\begin{align*}
    \cost(M_t) & \leq \cost_T(\Mcal_t).
\end{align*}
Taking expectation over the randomization of the algorithm,
\begin{align*}
    \expct{\cost(M_t)} & \leq \expct{ \cost_T(\Mcal_t)}
\end{align*}
which combined with $\expct{\cost_T( \Mcal_T)} \leq \Ocal(\log k) \cdot \cost(\Mcal_T)$, proves that $\expct{\cost(M_t)} \leq \Ocal(\log k) \cdot \cost(\Mcal_t)$.
\end{proof}

\subsection{Dynamic Online Matching on an HST}
\label{sec:dynamic_HST}

We describe the algorithm in Figure~\ref{fig:alg_dynamic_matching}. In a nutshell, to ensure optimality, the algorithm ensures that for all nodes $v$ of the tree, the number of clients in the subtree rooted at $v$ who are matched at a level equal or higher than the level of $v$ is given by the discrepancy between number of clients and servers in the subtree. 

\begin{figure}[t]
    \centering
\fbox{\parbox{\textwidth}{
\textbf{Algorithm $3$: Nearest Match}\\

{\it (i)} On arrival of client $c_t$ at time $t$ and leaf $x$:
\begin{enumerate}
\item $level \leftarrow 1$   
\item While there exists an unmatched client
\begin{enumerate}
    \item If the subtree of unmatched client rooted at level $level$ has a free server then match the unmatched client to it
    \item Else, if the subtree of unmatched client rooted at level $level$ has a server $s$ currently matched to a client $c$ with level  $level' > level$, then match the currently unmatched client to server $s$ and create an unmatched client $c$; set $level \leftarrow level'$
    \item Else, $level \leftarrow level + 1$
\end{enumerate}
\end{enumerate}

{\it (ii)} On arrival of free server $s_t$ at time $t$ and leaf $x$:
\begin{enumerate}
\item $level \leftarrow 1$   
\item While $level < D$
\begin{enumerate}
    \item If the subtree of the new free server rooted at level $level$ has a client $c$ currently matched to a server $s$ with level  $level' > level$, then match the free server to $c$ and create a new free server $s$; set $level \leftarrow level'$
    \item Else, $level \leftarrow level + 1$
\end{enumerate}
\end{enumerate}

{\it (iii)} On departure of a server at time $t$:
\begin{enumerate}
    \item Insert its currently matched client as a new client and run the first subroutine
\end{enumerate}

{\it (iv)} On departure of a client at time $t$:
\begin{enumerate}
    \item Insert its currently matched server as a new free server and run the second subroutine
\end{enumerate}
}}
    \caption{Nearest Match algorithm for Dynamic matching in HSTs}
    \label{fig:alg_dynamic_matching}
\end{figure}

==> line-metric.tex <==
\section{Online Matching on the Line metric}
\label{sec:line}

In this section we focus on the special case of a line metric. That is, for all points $x \in \Xcal$, we associate a location $\ell:\Xcal \to \RR$, and $d(x,y) = |\ell(x) - \ell(y)|$. We will use $\ell(c)$ and $\ell(s)$ as shorthand for the location of the client $c$ and server $s$ respectively. 

A first attempt at maintain an approximately optimal matching with low recourse is to always maintain the optimal matching. A simple example shows that this can incur a large recourse. Before we present the example, we observe that if we maintain the optimal matching, the set of servers used for clients $C_t$ by time $t$ must be the servers used by Permutation algorithm in $\Mcal_t$. Next, since the metric is line, we can order the clients and servers in $\Mcal_t$ in increasing order of their locations. Then, an optimal matching is a {\it parentheses matching}.

\begin{definition}[Parentheses matching]
A matching of a set of clients $C$ to a set of servers $S$ ($|C|=|S|$) on a line metric with location function $\ell(\cdot)$ is a Parentheses matching if and only if there exists an ordering of $C \union S$ where the clients and servers appear in increasing order of their locations, and a client $c$ and server $s$ are matched if and only if the number of clients that precede (succeed) both $c$ and $s$ equals the number of servers that precede (succeed) both $c$ and $s$.
\end{definition}

The name comes from the following interpretation: Imagine sweeping the list of clients and servers in the optimal matching from left to right and creating a matching as follows: Imagine placing an opening parenthesis at the leftmost node which is as yet unmatched. If the next node encountered is of the same type (server or client) as the currently unmatched node, then we place another opening parenthesis at its place, otherwise we place a closing parenthesis matching it to the last opening parenthesis placed. Clearly at any time in this sweep, there can be unmatched node of only one type. Further, the matching obeys a laminar (nested or disjoint) structure. Returning to the example: consider a sequence of arrivals such that the ordered list of clients an servers in $\Mcal_1$ is $(c_1, s_1)$; in $\Mcal_2$ is $(s_2, c_1, s_1, c_2)$; in $\Mcal_3$ is $(c_3, s_2, c_1, s_1, c_2, s_3)$, and so on. That is, the new clients and servers are added at the end of the list on alternating sides. In this case, the recourse at time $t$ to arrive at $\Mcal_t$ is $t$ for a final recourse of $n/2$ per client. 

The failure of the above naive algorithm motivates our approach. If we imagine a pair $(c,s)$ as an arc from client $c$ to server $s$, the pairs $(c_1, s_1)$, $(c_2, s_2)$, $(c_3, s_3)$ were alternating forward and backward arcs. Trying to update our matching when the new pair $(c_t, s_t)$ is either a forward or a backward arc led to a large recourse. In our proposed algorithm, we only fix a matching when the new $(c_t, s_t)$ pair is a backward arc. A forward $(c_t, s_t)$ pair is added as is creating a sub-optimal matching. 

Our algorithm, Farthest server, is given in Figure~\ref{fig:alg_farthest_server}. The main result of this section is the following:

\begin{theorem}
\label{thm:farthest_server_performance}
At all times $t$, the cost of the matching $M_t$ produced by Farthest Server algorithm (Figure~\ref{fig:alg_farthest_server}) satisfies $\cost(M_t) \leq 3 \cost(\Mcal_t)$. Further, the total number of recourse steps by time $t$ is at most $O(t \log(t))$. In other words, Farthest Server is $(3, \Ocal(\log n))$-competitive for the line metric.
\end{theorem}

In Section~\ref{sec:perf_farthest_server} we prove that the matching produced has a cost at most 3 times the optimal matching, and in Section~\ref{sec:recourse_farthest_server} we prove the bound on number of recourse steps.

\begin{figure}[t]
    \centering
\fbox{\parbox{\textwidth}{
\textbf{Algorithm $1$: Farthest Server}\\
At time $t$:
\begin{enumerate}
\item Let $s_t$ denote the server added by Permutation when client $c_t$ arrives. 
\item If $(c_t,s_t)$ is a forward arc add as it is. 
\item Else, consider all the clients between $c_t$ and $s_t$ that are currently matched via a forward arc. Let that set be $C_f$. Let $S_f$ be the set of servers matched to $C_f$. 
Let $A = C_f \cup S_f \cup \{c_t,s_t\} $. 
Initialize $list = \emptyset$ as the list of tentatively unmatched nodes.
\item Go over the clients and servers in $A$ from left to right, and match the clients and servers as follows: 
\begin{enumerate}
\item When at a server $s$: if $list$ is empty, add $s$ to $list$. Else, if the currently matched client of $s$ is in $list$, remove it and keep the old match of $s$. Else,  match $s$ to the client in $list$ whose currently matched server is the farthest (has largest $\ell()$) and remove this client from $list$. %If $c$ is there in the list, it gets preference over other clients if the current match of the server is unavailable.
\item When at a client $c$: If there is any server in $list$ (there can be at most 1), match the client to this server and remove the server from $list$. Else, add $c$ to $list$. 
\end{enumerate}
\end{enumerate}
}}
    \caption{Farthest Server algorithm for matching with recourse on a line metric}
    \label{fig:alg_farthest_server}
\end{figure}

\medskip




\subsection{Competitive ratio analysis}
\label{sec:perf_farthest_server}


% It suffices if we prove bound on the cost of reverse arcs. 
% Because, we can prove that the total cost of forward arcs is at most total cost of reverse arcs plus OPT. 
% Consider the matching between clients that are matched with forward arcs, and their respective servers using these forward arcs. 
% As all the arcs are in one direction, this matching is an optimal matching between these set of clients and servers.
% However, we can find a matching between these clients and servers of cost at most the sum of OPT and reverse arcs by taking symmetric difference of those two matchings. 
% Thus, the claim follows. 

% We have the following property that the ends of the "forward blocks" have no arcs crossing them, and thus have discrepancy zero. 

To ease the analysis, We introduce a second algorithm which produces a matching with the same cost as the Farthest Server algorithm (but at a potentially higher recourse cost). We then prove that the matching produced by this new algorithm has a competitive ratio of 3, thus implying that the original algorithm also produces a matching with cost at most 3 times the optimal matching. 

\medskip

\begin{figure}[t]
    \centering
\fbox{\parbox{\textwidth}{
\textbf{Algorithm $2$: Recursive farthest server}\\
At time $t$:
\begin{enumerate}
\item Let $s_t$ denote the server added by Permutation when client $c_t$ arrives. 
\item If $(c_t,s_t)$ is a forward arc add as it is. 
\item Else let $a$ be the current backward arc $(s_t,c_t)$.
\item While a currently matched $(c',s')$ pair is a forward arc intersecting $a$:
\begin{enumerate}
    \item Let $b=(c',s')$ be such a forward arc with the  rightmost server $s'$ intersecting $a=(s_t,c_t)$: $\ell(s_t) \leq \ell(s') \leq \ell(c_t)$ 
    \item Rematch $s'$ to $c_t$
    \item $a \longleftarrow (s_t,c')$
\end{enumerate}
\item Match the client and server in the arc $a$
\end{enumerate}
}}
    \caption{Recursive Farthest Server algorithm for cost analysis of Farthest Server algorithm}
    \label{fig:alg_recursive_farthest_server}
\end{figure}


\begin{lemma}
\label{lem:shrink}
Suppose the match of a server $s$ is changed from $c_1$ to $c_2$ during the course of the Algorithm $2$. Then, $\ell(c_2) \geq \ell(c_1)$. 
\end{lemma}
\begin{proof}
Note that once a server is matched by a backward arc, it is not going to change its match from that point onward. Hence, we can assume that $c_1$ to $s$ is a forward arc. 
Also note that in a single iteration of the algorithm, each server is rematched at most once in the recursive step. 

Consider the iteration of Algorithm $2$ in which we rematch server $s$ from $c_1$ to $c_2$.  
Let $(s',c')$ be the starting arc that was obtained from permutation.  
During the recursive step of the iteration, $c_1,s$ intersected with backward arc $c_2,s'$, and thus the match of $s$ is changed from $c_1$ to $c_2$. 
This implies that $c_2$ is to the right of $c_1$ since otherwise the two arcs would not have intersected. 
\end{proof}

% \begin{lemma}
% At the end of each iteration of Algorithm $2$, if a forward arc and a backward arc intersect, then the backward arc's client has arrived before the forward arc's client.
% \end{lemma}
% \begin{proof}
% %Consider an iteration in which $x(c) > x(s)$. All the reverse arcs added during the process do not intersect with any forward arcs. 
% \end{proof}


\begin{definition}[Segment]
A segment is defined as the region between consecutive nodes in $C_t \cup S_t$ for a given time $t$. 
\end{definition}
We slightly misuse this definition to say that ``segment of an arc'' meaning the portion of arc in a segment. 

\begin{lemma}
At any given point of time, the number of forward arcs crossing a segment remains same independent of whether Algorithm $1$ or $2$ is followed. 
\end{lemma}
\begin{proof}
We prove this inductively on the number of client server pairs added by the algorithms. Permutation algorithm outputs the new server independent of how we rematch existing clients and servers. When a new arc given by Permutation is a forward arc, both the algorithms add it as it is. 

Assume that the new arc given by permutation is a backward arc. 
Consider algorithm $2$. Let $C_o$ denote the set of clients in between $c_t$ and $s_t$. Let $S_o$ denote the set of servers matched to $C_o$ currently. Let $A = C_o \cup S_o \cup \{c_t,s_t\}$. The algorithm replaces existing matching between $C_o$, $S_o$ and $c_t,s_t$ with an optimal matching between clients and servers in $A$. This is because the reverse arcs added by the algorithm do not intersect with any forward arcs. Also note that the algorithm does not rematch any clients and servers outside $A$. 
Note that since all the arcs between $C_o \cup S_o$ are forward arcs, the existing matching between $C_o$ and $S_o$ is optimal as well. Thus, by discrepancy counting, the number of forward arcs in any segment outside $[\ell(s_t),\ell(c_t)]$ is unchanged. In segments between $\ell(s_t)$ and $\ell(c_t)$ where there are forward arcs already, the number of forward arcs decreases by one. 

However, by inductive claim, the segments where there are forward arcs is same when we are running Algorithm $1$ as well. In addition, algorithm $1$ also finds optimal solution with the clients that have forward arcs added with $c_t$. 
%By the inductive claim, we can also conclude that the set of clients $C$ and the set of servers $S$ will also be the same for Algorithm $1$. 
Since the sections where the forward arcs are present is same for both the algorithms, both the algorithms perform identical changes of number of forward arcs in any segment. 
\end{proof}

\begin{corollary}
Competitive ratio of Algorithm $1$ (Farthest Server) and $2$ (Recursive Farthest Server) are the same. 
\end{corollary}

\begin{proof}
Since the number of forward arcs is same in any segment, by discrepancy counting, the number of backward arcs is also same. Thus, the total cost is same at any point for both the algorithms. 
\end{proof}

For a given forward arc, we define redundant and non redundant segments of an arc. 
\begin{definition}(Redundant arc segments)
\begin{enumerate}
\item Suppose that a client $c$ is matched to a server $s$ with a forward arc when $c$ arrives. 
Then, a segment in this arc is defined to be redundant if  after adding $c$ and $s$, the number of clients to the left of both $(c,s)$ is at most the number of servers in the optimal offline matching immediately after arrival of $c$. Else, it is called non redundant. 
\item If a new forward arc is added during an iteration in which we add a backward arc, then a segment in the new arc $(c',s)$ is defined to be redundant if and only if the corresponding segment is redundant in arc $(c,s)$, where $c$ is the client that $s$ is matched to before $c'$. 
\end{enumerate}
\end{definition}

Intuitively, redundant forward arc segments are the segments where our algorithm pays more cost compared to the optimal solution. Our algorithm pays more cost both for the redundant forward arcs, and also some of the existing backward arcs. For example, it is possible that in some segment, the Recursive Farthest Server algorithm results in $2$ forward arcs and $3$ backward arcs, whereas the optimal matching will only have one backward arc. Thus, we pay $4$ times the length of the segment in addition to the optimal cost for this segment. 

\begin{lemma}
\label{lem:suffix}
If a forward arc $a=(c,s)$ is added during an iteration, then in any suffix of $a$, the length of non redundant segments is at least the length of redundant segments. 
\end{lemma}

\begin{proof}
Let $A$ denote the set of clients and servers prior to adding $c$ and $s$. Let $x \in [\ell(c),\ell(s)]$. We are interested in the suffix $[x,\ell(s)]$ of the arc $c,s$. Introduce a virtual client $c'$ at $x$. Consider the optimal solution of $A \cup \{c',s\}$. Since we are following Permutation till before $c$ is added, the optimal cost of matching $A \cup \{c',s\}$ is at least the optimal cost of matching $A$.

Note that if we add $c'$ to $A$, Permutation might not choose $s$. However, irrespective of which client server pair we add, the optimal solution can only go up. If not, we can take a subset of the new matching ignoring the new client and get a solution of lower cost to the previous instance. 
Thus, obtaining a contradiction to the fact that Permutation maintains a solution that has minimum optimal solution at any point. 

When we add $c',s$ to $A$, the increase in cost of optimal matching occurs precisely at the segments where the number of clients to the left is greater than the number of servers (after adding $c',s$). And in other segments in $[x,\ell(s)]$, the cost paid by the optimal matching decreases. 
However, this exactly corresponds to the redundancy and non-redundancy of the forward arc $c,s$ within segments inside $[x,\ell(s)]$. The segments where cost of optimal matching increases are the ones which are non-redundant, and the segments where the cost of optimal matching decreases are the ones which are redundant. 
\end{proof}

\begin{lemma}
\label{lem:redundant-bound}
The total cost of redundant forward segments is at most the total cost of non redundant forward segments. 
\end{lemma}
\begin{proof}
By summing up over each arc, using Lemma~\ref{lem:suffix}.
\end{proof}

\begin{lemma}
\label{lem:redundant}
At any point of time, in any segment, the number of redundant forward arcs is equal to the minimum of forward and backward arcs crossing this segment. 
\end{lemma}
\begin{proof}
We prove the following inductively on the number of client-server pairs added:
\begin{enumerate}
    \item In any segment, the number of redundant forward arcs is equal to the minimum of number of forward and backward arcs crossing this segment. 
    \item In any segment, if a redundant and non-redundant arc intersect, then the server of non-redundant arc is to the right of the server of redundant arc. (Assume that no two servers have the same $\ell(\cdot)$)
\end{enumerate}
Let $c,s$ be the client server pair given by Permutation.
Consider the two cases, adding a forward arc and a backward arc. 
\begin{enumerate}
    \item Suppose that $s$ is to the right of $c$ i.e. the case when we add the forward arc directly. 
    If in a segment between $c$ and $s$, there are fewer forward arcs than backward arcs prior to adding $c$ and $s$, we mark that segment as a redundant segment. Observe that this ensures that in those segments, redundant forward arc count increases, and is equal to the minimum of forward and backward arcs crossing the segment. 
    In segments where the number of forward arcs is at least the number of backward arcs prior to adding $c$ and $s$, the segment is non-redundant. In this case, the minimum of forward and backward arcs does not increase, and thus this ensures that the claim continues to remain valid. 

    For the second claim: If in a segment, the new arc is marked redundant, then all the forward arcs in that segment are redundant. If in a segment, the new arc is marked non-redundant, we need to show that the new server is to the right of any server whose arc is marked redundant. This follows directly from the fact that an unmatched server cannot be present in the middle of an arc (by optimality of the Permutation algorithm), and hence, $s$ is to the right of server of any forward arc that intersects $c,s$. 

    \item Suppose that $s$ is to the left of $c$ i.e. the case when we recursively add backward arc(s). 
    From Lemma~\ref{lem:shrink}, we know that the forward arcs corresponding to a server only shorten. Thus, second claim trivially follows. 
    
    Recall that the algorithm deletes a forward arc from the segments between $c$ and $s$ where there is at least one forward arc. 
    If the number of forward arcs in a segment is at most the number of backward arcs, then all of them are redundant arcs, and we delete one redundant one. The equation of claim $1$ still follows. 
    Thus, it remains to show that if there are both non-redundant and redundant arcs in a segment, our algorithm deletes the non-redundant one. 
    We use claim $2$ here. If there are both redundant and non-redundant arcs in a segment, note that the server corresponding to the non-redundant arc is to the right of the server corresponding to the redundant arc. 
    
    Also recall that there is at most one forward arc that is deleted from any segment. 
    If a redundant arc is deleted from a segment, when the arc is selected, it has the farthest server among all arcs that intersect the reverse arc. This combined with the above fact implies that if a redundant arc is deleted from a segment, then there is no non-redundant arc in that segment. Thus, if there are both redundant and non-redundant forward arcs inside a segment, our algorithm deletes the non-redundant arc. 
\end{enumerate}
\end{proof}

\begin{theorem}
At any point of time, the cost of the matching of Algorithm $2$ (Recursive Farthest server) is at most $3$ times the cost of the optimal offline matching. 
\end{theorem}
\begin{proof}
The set of clients and servers matched by the optimal offline matching $\Mcal_t$, as well as the algorithms 1 and 2 are identical, and therefore the the same set of segments are induced by looking at consecutive nodes in the matching. We decompose the total cost of the optimal matching $\Mcal_t$ and that returned by Algorithm 2 over these segments. 

For a given matching $M$, we denote the total cost of non-redundant forward arcs as $\cost(M, NF)$, and the total cost of redundant forward arcs as $\cost(M, RF)$. Similarly, $\cost(M,NB)$ and $\cost(M,RB)$ denote the cost of non-redundant and redundant backward arcs, respectively. 

The optimal offline matching $\Mcal_t$ only has non-redundant arcs: 
\begin{align*}
    \cost(\Mcal_t) &= \cost(\Mcal_t, NF) + \cost(\Mcal_t , NB).
\end{align*}
Writing out the cost of the potentially suboptimal matching produced by Algorithm 2:
\begin{align*}
    \cost(M_t) &= \cost(M_t, RF) + \cost(M_t, RB) + \cost(M_t, NF) + \cost(M_t , NB) \\
    \intertext{Since the redundant forward and redundant backward arc segments come in pairs by Lemma~\ref{lem:redundant},}
    &= 2 \cost(M_t, RF) + \cost(M_t, NF) + \cost(M_t, NB)
    \intertext{and from Lemma~\ref{lem:redundant-bound} bounding the cost of redundant forward arc segments by non-redundant forward arc segments}
        & \leq 2 \cdot \cost(M_t, NF) + \cost(M_t, NF) + \cost(M_t, NB) \\
        & \leq 3 \cdot \cost(\Mcal_t, NF) + \cost(\Mcal_t, NB) \\
        & \leq 3 \cdot \cost(\Mcal_t).
\end{align*}
\end{proof}

\subsection{Recourse of the Algorithm}
\label{sec:recourse_farthest_server}
We begin with some lemmas needed for the final result.
\begin{lemma}
\label{lem:reverse-disjoint}
After every iteration, the reverse arcs added do not intersect with any forward arcs. 
\end{lemma}
\begin{proof}
Our solution is the optimal one within set $A$ because the cost we pay in any segment between two consecutive nodes is equal to the discrepancy of clients and servers. 
As a consequence of optimality, there are no intersection between reverse and forward arcs. 
\end{proof}

It turns out that the farthest recourse matching within $A$ gives a key property of the new edges.
\begin{lemma}
\label{lem:disjoint}
In a single iteration (adding a new client), the new arcs added by the algorithm are disjoint. 
\end{lemma}

We state a couple of technical lemmas in order to prove Lemma~\ref{lem:disjoint}. 

\begin{lemma}
\label{lem:shorten}
If $c$ is a client that is currently matched to a server $s$ by a forward arc, and gets rematched to server $s'$ during a single iteration of the algorithm. Then $s'$ is to the left of $s$. 
\end{lemma}
\begin{proof}
Suppose for the sake of contradiction that $s'$ is to the right of $s$. 
Note that once a client gets matched via a reverse arc, the algorithm does not rematch it. 
Thus, $c$ is to the left of $s$, and thus to the left of $s'$. 
As $c$ is in the list of clients when the algorithm considers $s'$, it is in the list when the algorithm considers $s$ as well. Thus, $s$ should not have been rematched. 
\end{proof}
\begin{lemma}
\label{lem:unique-server}
At any point during a single iteration, the number of servers yet unconsidered by the algorithm but whose client has been rematched to a different server is at most one.  
\end{lemma}
\begin{proof}
Fix the iteration as adding a reverse arc $c,s$. We will prove the Lemma by inducting on the number of nodes (union of clients and servers) visited by the algorithm in the iteration. 
Let $c'$ be the client matched with $s$ by the algorithm. 
Note that $c'$ is the second node visited by the algorithm. 
At this point, the server $s'$ that is originally matched to $c'$ is the only server satisfying the above property. 
This covers the base case of the induction. 

Suppose that the property is true till we add a new node $p$. 
If $p$ is a client, adding $p$ to the list or matching it with a server to the left of it does not rematch any clients of servers yet unconsidered by the algorithm. 
If $p$ is a server, if it is the unique server whose client has already been rematched, we now get a new server added to $list$. 
If it has not lost its client yet, the set of servers whose clients are lost does not change (by design of the algorithm). 
\end{proof}

\begin{proof}(Of Lemma~\ref{lem:disjoint}) Let $s$ be an arbitrary server that was rematched during an iteration of the algorithm such that $s$ is not the new server added by the Permutation algorithm. 
Let $s_1$ be the server nearest to $s$ on left side that is rematched. 
Note that such a server exists since $s$ is not the left most server rematched, as the newly added server is the leftmost server rematched. 
Let $c$ be the client matched to $s$ before rematching. 
We prove that the new matches of $s$ and $s_1$ are disjoint. 
Applying this argument to all the servers other than the newly added server, we have proved the lemma. 

We consider two cases separately. 
\begin{enumerate}
\item $s_1$ now has a forward arc. 
First, we claim that $c$ is the client that $s_1$ is rematched to, after the end of iteration. 
Suppose for contradiction that $s_1$ is rematched to $c' \neq c$. 
Note that as $s$ is rematched, $c$ should be rematched too. As $s_1$ is the closest server on left to $s$ that is rematched, $c$ should be rematched to a server to the left of $s_1$. In other words, just after when we consider $s_1$ in the course of algorithm, $s$ is a server whose client is already lost. However, note that the server originally matched to $c'$ has also now lost its client. Thus, we arrive at a contradiction to Lemma~\ref{lem:unique-server}.

Let $c_1$ be the client that $s$ is rematched to. We claim that $c_1$ is to the right of $s_1$ which proves that the new arcs adjacent to $s$ and $s_1$ are disjoint. 
Suppose that $c_1$ is to the left of $s_1$. 
From Lemma~\ref{lem:shorten}, we know that $c_1$'s original match is to the right of $s$. 
Thus, when the algorithm is considering $s_1$, it would match $s_1$ with $c_1$ rather than $c$, since $c_1$ has ``farthest server''. 
\item $s_1$ now has a reverse arc. This case follows from the fact that the reverse arcs that we added don't intersect with any forward arcs. 
\end{enumerate}
\end{proof}

For a client $c$ that is currently matched by a forward arc to server $s$, its server-set is defined as the set of servers $s'$ such that $\ell(c) \leq \ell(s')\leq \ell(s)$. 

Lemma~\ref{lem:disjoint} also implies another simple but useful property:
\begin{lemma}
\label{lem:server-closer}
If a server $s$ has changed its match from $c_1$ to $c_2$, both using forward arcs, then $c_2$ lies to the right of $c_1$ i.e. $\ell(c_2) \geq \ell(c_1)$.
\end{lemma}
\begin{proof}
Suppose in a particular iteration, the server $s$ has changed its match from $c_1$ to $c_2$, and $c_2$ is to the left of $c_1$. 
As $c_1$ lies in between $c_2$ and $s$, the new arc of $c_1$ intersects $c_2$ and $s$ which directly contradicts Lemma~\ref{lem:disjoint}.
\end{proof}

\begin{theorem}
\label{thm:recourse}
The total recourse of Farthest Server algorithm is at most $O(n\log(n))$
\end{theorem}

\begin{proof}
Note that once a client is matched by a reverse arc, it is not going to get rematched later. 
Thus, we are only interested in bounding the number of rematches that match forward arcs to forward arcs. 
\smallskip

For a node (either client or server) $z$, let us define a ``length'' $len(z)$ parameter which is equal to the number of nodes (all nodes which are part of the eventual matching after all $n$ clients have arrived) lying strictly inside the arc of $z$. 
Therefore, before start of the algorithm, the $len$ value of every node is at most $2n$. We now define the level of node $z$ as $\floor{\log len(z)}$ so that the total initial level of all the nodes is at most $2n (1+\log n)$. Suppose that a client $c$ is currently matched to $s$ by using a forward arc, and in a iteration gets rematched to $s'$ and $s$ gets rematched to $c'$ both again using forward arcs. At least one of $len(c)$ or $len(s)$ should have decreased by at least factor of $2$. And therefore the total level of $c$ and $s$ at least decreases by 1. In other words, on every rematch, the total level decreases by at least 1, which together with the bound on total initial level gives the number of such rematches to be at most $2n ( 1+\log n)$.
If at least one of $c$ or $s$ gets rematched by a reverse arc, its match does not change from then on. 
Thus, the number of these type of rematches are at most $2n$.
Thus, in total, the recourse of the algorithm is $O(n \log n)$.
\end{proof}



==> line.tex <==
\section{Online Matching on the Line metric}
\label{sec:line}

In this section we focus on the special case of a line metric. That is, for all points $x \in \Xcal$, we associate a location $\ell:\Xcal \to \RR$, and $d(x,y) = |\ell(x) - \ell(y)|$. We will use $\ell(c)$ and $\ell(s)$ as shorthand for the location of the client $c$ and server $s$ respectively. 

A first attempt at maintain an approximately optimal matching with low recourse is to always maintain the optimal matching. A simple example shows that this can incur a large recourse. 
Before we present the example, we observe that if we maintain the optimal matching, the set of servers used for clients $C_t$ by time $t$ must be the servers used by \permutation algorithm in $\Mcal_t$. Next, since the metric is line, we can order the clients and servers in $\Mcal_t$ in increasing order of their locations. Then, one possible optimal matching is the {\it parentheses matching}.

\begin{definition}[Parentheses matching]
A matching of a set of clients $C$ to a set of servers $S$ ($|C|=|S|$) on a line metric with location function $\ell(\cdot)$ is a Parentheses matching if and only if there exists an ordering of $C \union S$ where the clients and servers appear in increasing order of their locations, and a client $c$ and server $s$ are matched if and only if the number of clients that precede (succeed) both $c$ and $s$ equals the number of servers that precede (succeed) both $c$ and $s$. Or equivalently, the number of clients lying between $c$ and $s$ is equal to the number of servers lying between $c$ and $s$.
\end{definition}

The name comes from the following interpretation: Imagine sweeping the list of clients and servers in the optimal matching from left to right and creating a matching as follows: we place an opening parenthesis at the leftmost node which is as yet unmatched. If the next node encountered is of the same type (server or client) as the currently unmatched node, then we place another opening parenthesis at its place, otherwise we place a closing parenthesis matching it to the last opening parenthesis placed. Clearly at any time in this sweep, there can be unmatched nodes of only one type. Further, the matching obeys a {\it laminar} (nested or disjoint) structure. Returning to the example: consider a sequence of arrivals such that the ordered list of clients and servers in $\Mcal_1$ is $(c_1, s_1)$; in $\Mcal_2$ is $(s_2, c_1, s_1, c_2)$; in $\Mcal_3$ is $(c_3, s_2, c_1, s_1, c_2, s_3)$, and so on. That is, the new clients and servers are added at the end of the list on alternating sides. In this case, the recourse at time $t$ to arrive at $\Mcal_t$ is $t$ for a final recourse of $(k-1)/2$ per client. 
\todo{Phrase this example in terms of just clients arriving}

The failure of the above naive algorithm motivates our approach. If we imagine a pair $(c,s)$ as an arc from client $c$ to server $s$, the pairs $(c_1, s_1)$, $(c_2, s_2)$, $(c_3, s_3)$ were alternating forward and backward arcs. Trying to update our matching when the new pair $(c_t, s_t)$ is either a forward or a backward arc led to a large recourse. In our proposed algorithm, we only change the matching when the new $(c_t, s_t)$ pair is a backward arc. A forward $(c_t, s_t)$ pair is added as is, creating a sub-optimal matching. 

Our algorithm, Farthest server, is given in Algorithm~\ref{alg:farthest_server}. The main result of this section is the following:

\begin{theorem}
\label{thm:farthest_server_performance}
At all times $t$, the cost of the matching $M_t$ produced by Farthest Server algorithm (Algorithm~\ref{alg:farthest_server}) satisfies $\cost(M_t) \leq 3 \cost(\Mcal_t)$. Further, the total number of recourse steps by time $t$ is at most $O(t \log(t))$. In other words, Farthest Server is $(3, \Ocal(\log k))$-competitive for the line metric.
\end{theorem}

In Section~\ref{sec:perf_farthest_server} we prove that the matching produced has a cost at most 3 times the optimal matching, and in Section~\ref{sec:recourse_farthest_server} we prove the bound on number of recourse steps.

\begin{algorithm}
	\caption{Farthest Server}
\label{alg:farthest_server}
		\begin{algorithmic}[1]
		\For {each time $t$ ($c_t$ denoting the arriving client and $s_t$ the server added by \permutation ) }
		\If {$(c_t,s_t)$ is a forward arc}
		    \State {add $(c_t,s_t)$ as it is}
		\Else
		    \State {$C_f \leftarrow $ all clients between $c_t$ and $s_t$ that are currently matched via a forward arc}
		    \State $S_f \leftarrow $ the set of servers matched to $C_f$
		    \State $A \leftarrow C_f \cup S_f \cup \{c_t,s_t\} $
		    \State $list \leftarrow \emptyset$ \Comment {The list of tentatively unmatched nodes}
		\For {Each \textit{node} in $A$ (in left to right order)}
            \If {\textit{node} is server (denote by $s$) }
            \If {$list$ is empty}
            \State $list \leftarrow list \cup \{s\}$ 
            \Else 
            \State  \If {the currently matched client of $s$ is in $list$}
            \State remove the client and keep the old match of $s$ 
            \Else
            \State $c' \leftarrow$ client in $list$ with rightmost matched server
            \State match $s$ to $c'$ 
            \State $list \leftarrow list \backslash \{c'\}$. %If $c$ is there in the list, it gets preference over other clients if the current match of the server is unavailable.
            \EndIf
            \EndIf
            \Else {\ (\textit{node} is a client (denote by $c$))}
            \If {there is any server $s'$ in $list$ (there can be at most 1)}
                \State match $c$ to $s'$
                \State $list \leftarrow list \backslash \{s'\}$
            \Else
                \State $list \leftarrow list \cup \{c\}$
            \EndIf
            \EndIf
		\EndFor
		\EndIf
		\EndFor
	\end{algorithmic}
	%\end{center}
	\end{algorithm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
    \centering
\fbox{\parbox{\textwidth}{
\textbf{Algorithm $1$: Farthest Server}\\
At time $t$:
\begin{enumerate}
\item Let $s_t$ denote the server added by Permutation when client $c_t$ arrives. 
\item If $(c_t,s_t)$ is a forward arc add as it is. 
\item Else, consider all the clients between $c_t$ and $s_t$ that are currently matched via a forward arc. Let that set be $C_f$. Let $S_f$ be the set of servers matched to $C_f$. 
Let $A = C_f \cup S_f \cup \{c_t,s_t\} $. 
Initialize $list = \emptyset$ as the list of tentatively unmatched nodes.
\item Go over the clients and servers in $A$ from left to right, and match the clients and servers as follows: 
\begin{enumerate}
\item When at a server $s$: if $list$ is empty, add $s$ to $list$. Else, if the currently matched client of $s$ is in $list$, remove it and keep the old match of $s$. Else,  match $s$ to the client in $list$ whose currently matched server is the farthest (has largest $\ell()$) and remove this client from $list$. %If $c$ is there in the list, it gets preference over other clients if the current match of the server is unavailable.
\item When at a client $c$: If there is any server in $list$ (there can be at most 1), match the client to this server and remove the server from $list$. Else, add $c$ to $list$. 
\end{enumerate}
\end{enumerate}
}}
    \caption{Farthest Server algorithm for matching with recourse on a line metric}
    \label{fig:alg_farthest_server}
\end{figure}

\medskip
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\subsection{Competitive ratio analysis}
\label{sec:perf_farthest_server}


% It suffices if we prove bound on the cost of reverse arcs. 
% Because, we can prove that the total cost of forward arcs is at most total cost of reverse arcs plus OPT. 
% Consider the matching between clients that are matched with forward arcs, and their respective servers using these forward arcs. 
% As all the arcs are in one direction, this matching is an optimal matching between these set of clients and servers.
% However, we can find a matching between these clients and servers of cost at most the sum of OPT and reverse arcs by taking symmetric difference of those two matchings. 
% Thus, the claim follows. 

% We have the following property that the ends of the "forward blocks" have no arcs crossing them, and thus have discrepancy zero. 

To ease the analysis, We introduce a second algorithm which produces a matching with the same cost as the Farthest Server algorithm (but at a potentially higher recourse cost). We then prove that the matching produced by this new algorithm has a competitive ratio of 3, thus implying that the original algorithm also produces a matching with cost at most 3 times the optimal matching. 

\medskip

\begin{algorithm}
	\caption{Recursive Farthest Server}
\label{alg:recursive_farthest_server}
		\begin{algorithmic}[1]
		\For {each time $t$ ($c_t$ denoting the arriving client and $s_t$ the server added by \permutation ) }
		\If {$(c_t,s_t)$ is a forward arc}
		    \State {add $(c_t,s_t)$ as it is}
		\Else
		    \State $a \leftarrow (s_t, c_t) $
		    \Comment {current forward arc}
		    \While {a currently matched $(c',s')$ pair is a forward arc intersecting $a = (s,c)$}
		        \State $b \leftarrow (c',s')$ be such a forward arc with the rightmost server $s'$ intersecting $a$: $\ell(s) \leq \ell(s') \leq \ell(c)$
		        \State Rematch $s'$ to $c$
		        \State $a\leftarrow (s,c')$ 
		    \EndWhile
		    \State Match the client and server in the arc $a$
		    \EndIf
		    \EndFor
	\end{algorithmic}
	%\end{center}
	\end{algorithm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
    \centering
\fbox{\parbox{\textwidth}{
\textbf{Algorithm $2$: Recursive farthest server}\\
At time $t$:
\begin{enumerate}
\item Let $s_t$ denote the server added by Permutation when client $c_t$ arrives. 
\item If $(c_t,s_t)$ is a forward arc add as it is. 
\item Else let $a$ be the current backward arc $(s_t,c_t)$.
\item While a currently matched $(c',s')$ pair is a forward arc intersecting $a$:
\begin{enumerate}
    \item Let $b=(c',s')$ be such a forward arc with the  rightmost server $s'$ intersecting $a=(s_t,c_t)$: $\ell(s_t) \leq \ell(s') \leq \ell(c_t)$ 
    \item Rematch $s'$ to $c_t$
    \item $a \longleftarrow (s_t,c')$
\end{enumerate}
\item Match the client and server in the arc $a$
\end{enumerate}
}}
    \caption{Recursive Farthest Server algorithm for cost analysis of Farthest Server algorithm}
    \label{fig:alg_recursive_farthest_server}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{comment}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%



% \begin{lemma}
% At the end of each iteration of Algorithm $2$, if a forward arc and a backward arc intersect, then the backward arc's client has arrived before the forward arc's client.
% \end{lemma}
% \begin{proof}
% %Consider an iteration in which $x(c) > x(s)$. All the reverse arcs added during the process do not intersect with any forward arcs. 
% \end{proof}


\begin{definition}[Segment]
A segment is defined as the region between consecutive nodes in $C_t \cup S_t$ for a given time $t$. 
\end{definition}
We slightly misuse this definition to say that ``segment of an arc'' meaning the portion of arc in a segment. 

\begin{lemma}
At any given point of time, the number of forward arcs crossing a segment remains same independent of whether Algorithm $1$ or $2$ is followed. 
\end{lemma}
\begin{proof}
We prove this inductively on the number of client server pairs added by the algorithms. Permutation algorithm outputs the new server independent of how we rematch existing clients and servers. When a new arc given by Permutation is a forward arc, both the algorithms add it as it is. 

Assume that the new arc given by permutation is a backward arc. 
Consider algorithm $2$. Let $C_o$ denote the set of clients in between $c_t$ and $s_t$. Let $S_o$ denote the set of servers matched to $C_o$ currently. Let $A = C_o \cup S_o \cup \{c_t,s_t\}$. The algorithm replaces existing matching between $C_o$, $S_o$ and $c_t,s_t$ with an optimal matching between clients and servers in $A$. This is because the reverse arcs added by the algorithm do not intersect with any forward arcs. Also note that the algorithm does not rematch any clients and servers outside $A$. 
Note that since all the arcs between $C_o \cup S_o$ are forward arcs, the existing matching between $C_o$ and $S_o$ is optimal as well. Thus, by discrepancy counting, the number of forward arcs in any segment outside $[\ell(s_t),\ell(c_t)]$ is unchanged. In segments between $\ell(s_t)$ and $\ell(c_t)$ where there are forward arcs already, the number of forward arcs decreases by one. 

However, by inductive claim, the segments where there are forward arcs is same when we are running Algorithm $1$ as well. In addition, algorithm $1$ also finds optimal solution with the clients that have forward arcs added with $c_t$. 
%By the inductive claim, we can also conclude that the set of clients $C$ and the set of servers $S$ will also be the same for Algorithm $1$. 
Since the sections where the forward arcs are present is same for both the algorithms, both the algorithms perform identical changes of number of forward arcs in any segment. 
\end{proof}

\begin{corollary}
Competitive ratio of Algorithm $1$ (Farthest Server) and $2$ (Recursive Farthest Server) are the same. 
\end{corollary}

\begin{proof}
Since the number of forward arcs is same in any segment, by discrepancy counting, the number of backward arcs is also same. Thus, the total cost is same at any point for both the algorithms. 
\end{proof}
We start competitive ratio analysis of the algorithm by a simple, yet crucial lemma.

\begin{lemma}
\label{lem:shrink}
Suppose the match of a server $s$ is changed from $c_1$ to $c_2$ during the course of the Algorithm $2$. Then, $\ell(c_2) \geq \ell(c_1)$. 
\end{lemma}
\begin{proof}
Note that once a server is matched by a backward arc, it is not going to change its match from that point onward. Hence, we can assume that $c_1$ to $s$ is a forward arc. 
Also note that in a single iteration of the algorithm, each server is rematched at most once in the recursive step. 

Consider the iteration of Algorithm $2$ in which we rematch server $s$ from $c_1$ to $c_2$.  
Let $(s',c')$ be the starting arc that was obtained from permutation.  
During the recursive step of the iteration, $c_1,s$ intersected with backward arc $c_2,s'$, and thus the match of $s$ is changed from $c_1$ to $c_2$. 
This implies that $c_2$ is to the right of $c_1$ since otherwise the two arcs would not have intersected in the first place.
\end{proof}


For a given forward arc, we define redundant and non redundant segments of an arc. 
\begin{definition}(Redundant arc segments)
\begin{enumerate}
\item Suppose in an iteration of the algorithm, that a client $c$ is matched to a server $s$ with a forward arc when $c$ arrives. 
Then, a segment $(u,v), \ell(u)< \ell(v)$ in this arc is defined to be redundant if  after adding $c$ and $s$, the number of clients arrived so far to the left of $u$ is at most the number of servers used so far to the left of $u$. Else, it is called non redundant. 
\item If a new forward arc $(c',s)$ is added during an iteration in which we add a backward arc, then a segment in the new arc is defined to be redundant if and only if the corresponding segment is redundant in arc $(c,s)$, where $c$ is the client that $s$ is matched to before $c'$. 
Note that this definition makes sense because~\Cref{lem:shrink} implies that $c$ is guaranteed to be on the left of $c'$.
\end{enumerate}
\end{definition}

Intuitively, redundant forward arc segments are the segments where our algorithm pays more cost compared to the optimal solution. Our algorithm pays more cost both for the redundant forward arcs, and also some of the existing backward arcs. For example, it is possible that in some segment, the Recursive Farthest Server algorithm results in $2$ forward arcs and $3$ backward arcs, whereas the optimal matching will only have one backward arc. Thus, we pay $4$ times the length of the segment in addition to the optimal cost for this segment. 

\input{redundant-figure.tex}

\begin{lemma}
\label{lem:suffix}
If a forward arc $a=(c,s)$ is added during an iteration, then in any suffix of $a$, the length of non redundant segments is at least the length of redundant segments. 
\end{lemma}

\begin{proof}
Let $A$ denote the set of clients and servers prior to adding $c$ and $s$. Let $x \in [\ell(c),\ell(s)]$. We are interested in the suffix $[x,\ell(s)]$ of the arc $c,s$. Introduce a virtual client $c'$ at $x$. Consider the optimal solution of $A \cup \{c',s\}$. 
%Since we are following Permutation till before $c$ is added, the optimal cost of matching $A \cup \{c',s\}$ is at least the optimal cost of matching $A$.
We claim that the optimal cost of matching $A \cup \{c',s\}$ is at least the optimal cost of matching $A$.
Note that if we add $c'$ to $A$, \permutation might not choose to pair it with $s$. However, irrespective of which client server pair we add, the optimal solution can only go up. If not, we can take a subset of the new matching ignoring the new client and get a solution of lower cost to the previous instance. 
Thus, obtaining a contradiction to the fact that \permutation maintains a solution that is server-optimal.

When we add $\{c',s\}$ to $A$, the increase in cost of optimal matching occurs precisely at the segments where the number of clients to the left is greater than the number of servers (after adding $c',s$). And in other segments in $[x,\ell(s)]$, the cost paid by the optimal matching decreases. 
However, this exactly corresponds to the redundancy and non-redundancy of the forward arc $c,s$ within segments inside $[x,\ell(s)]$. The segments where cost of optimal matching increases are the ones which are non-redundant, and the segments where the cost of optimal matching decreases are the ones which are redundant. 
\end{proof}

\begin{lemma}
\label{lem:redundant-bound}
At any point, in our algorithm, the total cost of redundant forward segments is at most the total cost of non redundant forward segments. 
\end{lemma}
\begin{proof}
The proof follows by summing up over each arc using~\Cref{lem:suffix}.
\end{proof}

The redundant forward arc segments are defined so that they correspond to the segments in which there are both forward and backward arcs. 
We still need to argue that this property holds throughout the execution of the algorithm. 

\begin{lemma}
\label{lem:redundant}
At any point of time, in any segment, the number of redundant forward arcs is equal to the minimum of forward and backward arcs crossing this segment. 
\end{lemma}
\begin{proof}
We prove the following two claims inductively on the number of client-server pairs added:
\begin{enumerate}
    \item In any segment, the number of redundant forward arcs is equal to the minimum of number of forward and backward arcs crossing this segment. 
    \item In any segment, if a redundant and non-redundant forward arcs are present, then the server of non-redundant arc is to the right of the server of redundant arc. 
\end{enumerate}
Let $c,s$ be the client server pair given by \permutation.
Consider the two cases, adding a forward arc and a backward arc. 
\begin{enumerate}
    \item Suppose that $s$ is to the right of $c$ i.e. the case when we add the forward arc directly. 
    If in a segment between $c$ and $s$, there are fewer forward arcs than backward arcs prior to adding $c$ and $s$, we mark that segment as a redundant segment. Observe that this ensures that in those segments, redundant forward arc count increases, and is equal to the minimum of forward and backward arcs crossing the segment. 
    In segments where the number of forward arcs is at least the number of backward arcs prior to adding $c$ and $s$, the segment is non-redundant. In this case, the minimum of forward and backward arcs does not increase, and thus this ensures that the claim continues to remain valid. 

    For the second claim: If in a segment, the new arc is marked redundant, then all the forward arcs in that segment are redundant. If in a segment, the new arc is marked non-redundant, we need to show that the new server is to the right of any server whose arc is marked redundant. This follows directly from the fact that an unmatched server cannot be present in the middle of an arc (by optimality of the \permutation algorithm), and hence, $s$ is to the right of server of any forward arc that intersects $c,s$. 

    \item Suppose that $s$ is to the left of $c$ i.e. the case when we recursively add backward arc(s). 
    From Lemma~\ref{lem:shrink}, we know that the forward arcs corresponding to a server only shorten. Thus, second claim trivially follows. 
    
    The algorithm deletes a forward arc from the segments between $s$ and $c$ where there is at least one forward arc. 
    If the number of forward arcs in a segment is at most the number of backward arcs, then all of them are redundant arcs, and we delete one redundant one. The property of claim $1$ still holds. 
    Thus, it remains to show that if there are both non-redundant and redundant arcs in a segment, our algorithm deletes the non-redundant one. 
    We use claim $2$ here. If there are both redundant and non-redundant arcs in a segment, note that the server corresponding to the non-redundant arc is to the right of the server corresponding to the redundant arc. 
    
    Also recall that there is at most one forward arc that is deleted from any segment. 
    If a redundant arc is deleted from a segment, when the arc is selected, it has the farthest server among all arcs that intersect the reverse arc. This combined with the above fact implies that if a redundant arc is deleted from a segment, then there is no non-redundant arc in that segment. Thus, if there are both redundant and non-redundant forward arcs inside a segment, our algorithm deletes the non-redundant arc. 
\end{enumerate}
\end{proof}

\begin{theorem}
At any point of time, the cost of the matching of Algorithm~\ref{alg:recursive_farthest_server} (Recursive Farthest server) is at most $3$ times the cost of the optimal offline matching. 
\end{theorem}
\begin{proof}
The set of clients and servers matched by the optimal offline matching $\Mcal_t$, as well as the Algorithms~\ref{alg:farthest_server} and \ref{alg:recursive_farthest_server} are identical, and therefore the the same set of segments are induced by looking at consecutive nodes in the matching. We decompose the total cost of the optimal matching $\Mcal_t$ and that returned by Algorithm~\ref{alg:recursive_farthest_server} over these segments. 

For the sake of the competitive ratio analysis, we set some segments of backward arcs as redundant and the rest as non-redundant. 
In every segment, let an arbitrary set of backward arcs equal to the minimum of number of forward and backward arcs in this segment to be redundant, and the rest to be non-redundant. 
From~\Cref{lem:redundant}, the number of redundant backward arcs is equal to the number of redundant forward arcs in any segment. 

For a given matching $M$, we denote the total cost of non-redundant forward arcs as $\cost(M, NF)$, and the total cost of redundant forward arcs as $\cost(M, RF)$. Similarly, $\cost(M,NB)$ and $\cost(M,RB)$ denote the cost of non-redundant and redundant backward arcs, respectively. 

The optimal offline matching $\Mcal_t$ only has non-redundant arcs: 
\begin{align*}
    \cost(\Mcal_t) &= \cost(\Mcal_t, NF) + \cost(\Mcal_t , NB).
\end{align*}
Since~\Cref{alg:recursive_farthest_server} uses the same set of servers as the optimal solution, we obtain 
\begin{align*}
    \cost(M_t, NF) + \cost(M_t , NB) =\cost(\Mcal_t, NF) + \cost(\Mcal_t , NB).
\end{align*}
The cost of the matching maintained by our algorithm at any time can be bounded as follows:
\begin{align*}
    \cost(M_t) &= \cost(M_t, RF) + \cost(M_t, RB) + \cost(M_t, NF) + \cost(M_t , NB) \\
    \intertext{Since the redundant forward and redundant backward arc segments come in pairs by Lemma~\ref{lem:redundant},}
    &= 2 \cost(M_t, RF) + \cost(M_t, NF) + \cost(M_t, NB)
    \intertext{and from Lemma~\ref{lem:redundant-bound} bounding the cost of redundant forward arc segments by non-redundant forward arc segments}
        & \leq 2 \cdot \cost(M_t, NF) + \cost(M_t, NF) + \cost(M_t, NB) \\
        & \leq 3 \left( \cost(M_t, NF) + \cost(M_t, NB)\right) \\
        & = 3 \left( \cost(\Mcal_t, NF) + \cost(\Mcal_t, NB)\right) \\
        & \leq 3 \cdot \cost(\Mcal_t).
\end{align*}
\end{proof}

\subsection{Recourse of the Algorithm}
\label{sec:recourse_farthest_server}
We illustrate the fact that recursive farthest server algorithm can have bad recourse in the following example: 
\input{recourse-figure.tex}
In this instance, there are four clients $c_1,c_2,c_3$ and $c_4$, $\ell(c_1)<\ell(c_2)<\ell(c_3)<\ell(c_4)$ currently matched using forward arcs to $s_1, s_2,s_3$ and $s_4$ respectively such that $\ell(c_4)<\ell(s_1)<\ell(s_2)<\ell(s_3)<\ell(s_4)$.
A new client $c_5$ arrives to the right of $s_4$ and \permutation outputs $s_5$ to the left of $c_1$ as the server. 
Since the arc $(c_5,s_5)$ is backward, the algorithms try to fix the matching. 
The recursive farthest server i.e.~\Cref{alg:recursive_farthest_server} changes the matching completely to obtain $(c_2,s_1),(c_3,s_2),(c_4,s_3)$ as the new forward arcs, where as~\Cref{alg:farthest_server} changes only $c_4$'s matching and keeps $c_2$ and $c_3$ intact. 
If there are $k$ such forward arcs, and if $k$ backward arcs arrive, ~\Cref{alg:recursive_farthest_server} has a recourse of $\Omega(k^2)$ where as~\Cref{alg:farthest_server} has only $O(k)$ recourse. 

We begin the recourse analysis of~\Cref{alg:farthest_server} with simple lemma. 
\begin{lemma}
\label{lem:reverse-disjoint}
After every iteration, the reverse arcs added do not intersect with any forward arcs. 
\end{lemma}
\begin{proof}
Our solution is the optimal one within set $A$ because the cost we pay in any segment between two consecutive nodes is equal to the discrepancy of clients and servers. 
As a consequence of optimality, there are no intersection between reverse and forward arcs. 
\end{proof}

It turns out that the farthest recourse matching within $A$ gives a key property of the new edges.
\begin{lemma}
\label{lem:disjoint}
In a single iteration (adding a new client), the new arcs added by the algorithm are disjoint. 
\end{lemma}

We state a couple of technical lemmas in order to prove Lemma~\ref{lem:disjoint}. 

\begin{lemma}
\label{lem:shorten}
If $c$ is a client that is currently matched to a server $s$ by a forward arc, and gets rematched to server $s'$ during a single iteration of the algorithm. Then $s'$ is to the left of $s$. 
\end{lemma}
\begin{proof}
Suppose for the sake of contradiction that $s'$ is to the right of $s$. 
Note that once a client gets matched via a reverse arc, the algorithm does not rematch it. 
Thus, $c$ is to the left of $s$, and thus to the left of $s'$. 
As $c$ is in the list of clients when the algorithm considers $s'$, it is in the list when the algorithm considers $s$ as well. Thus, $s$ should not have been rematched. 
\end{proof}
\begin{lemma}
\label{lem:unique-server}
At any point during a single iteration, the number of servers yet unconsidered by the algorithm but whose client has been rematched to a different server is at most one.  
\end{lemma}
\begin{proof}
Fix the iteration as adding a reverse arc $c,s$. We will prove the Lemma by inducting on the number of nodes (union of clients and servers) visited by the algorithm in the iteration. 
Let $c'$ be the client matched with $s$ by the algorithm. 
Note that $c'$ is the second node visited by the algorithm. 
At this point, the server $s'$ that is originally matched to $c'$ is the only server satisfying the above property. 
This covers the base case of the induction. 

Suppose that the property is true till we add a new node $p$. 
If $p$ is a client, adding $p$ to the list or matching it with a server to the left of it does not rematch any clients of servers yet unconsidered by the algorithm. 
If $p$ is a server, if it is the unique server whose client has already been rematched, we now get a new server added to $list$. 
If it has not lost its client yet, the set of servers whose clients are lost does not change (by design of the algorithm). 
\end{proof}

\begin{proof}(Of Lemma~\ref{lem:disjoint}) Let $s$ be an arbitrary server that was rematched during an iteration of the algorithm such that $s$ is not the new server added by the Permutation algorithm. 
Let $s_1$ be the server nearest to $s$ on left side that is rematched. 
Note that such a server exists since $s$ is not the left most server rematched, as the newly added server is the leftmost server rematched. 
Let $c$ be the client matched to $s$ before rematching. 
We prove that the new matches of $s$ and $s_1$ are disjoint. 
Applying this argument to all the servers other than the newly added server, we have proved the lemma. 

We consider two cases separately. 
\begin{enumerate}
\item $s_1$ now has a forward arc. 
First, we claim that $c$ is the client that $s_1$ is rematched to, after the end of iteration. 
Suppose for contradiction that $s_1$ is rematched to $c' \neq c$. 
Note that as $s$ is rematched, $c$ should be rematched too. As $s_1$ is the closest server on left to $s$ that is rematched, $c$ should be rematched to a server to the left of $s_1$. In other words, just after when we consider $s_1$ in the course of algorithm, $s$ is a server whose client is already lost. However, note that the server originally matched to $c'$ has also now lost its client. Thus, we arrive at a contradiction to Lemma~\ref{lem:unique-server}.

Let $c_1$ be the client that $s$ is rematched to. We claim that $c_1$ is to the right of $s_1$ which proves that the new arcs adjacent to $s$ and $s_1$ are disjoint. 
Suppose that $c_1$ is to the left of $s_1$. 
From Lemma~\ref{lem:shorten}, we know that $c_1$'s original match is to the right of $s$. 
Thus, when the algorithm is considering $s_1$, it would match $s_1$ with $c_1$ rather than $c$, since $c_1$ has ``farthest server''. 
\item $s_1$ now has a reverse arc. This case follows from the fact that the reverse arcs that we added don't intersect with any forward arcs. 
\end{enumerate}
\end{proof}

For a client $c$ that is currently matched by a forward arc to server $s$, its server-set is defined as the set of servers $s'$ such that $\ell(c) \leq \ell(s')\leq \ell(s)$. 

Lemma~\ref{lem:disjoint} also implies another simple but useful property:
\begin{lemma}
\label{lem:server-closer}
If a server $s$ has changed its match from $c_1$ to $c_2$, both using forward arcs, then $c_2$ lies to the right of $c_1$ i.e. $\ell(c_2) \geq \ell(c_1)$.
\end{lemma}
\begin{proof}
Suppose in a particular iteration, the server $s$ has changed its match from $c_1$ to $c_2$, and $c_2$ is to the left of $c_1$. 
As $c_1$ lies in between $c_2$ and $s$, the new arc of $c_1$ intersects $c_2$ and $s$ which directly contradicts Lemma~\ref{lem:disjoint}.
\end{proof}

\begin{theorem}
\label{thm:recourse}
The total recourse of Farthest Server algorithm is at most $O(k\log(k))$
\end{theorem}

\begin{proof}
Note that once a client is matched by a reverse arc, it is not going to get rematched later. 
Thus, we are only interested in bounding the number of rematches that match forward arcs to forward arcs. 
\smallskip

For a node (either client or server) $z$, let us define a ``length'' $len(z)$ parameter which is equal to the number of nodes (all nodes which are part of the eventual matching after all $k$ clients have arrived) lying strictly inside the arc of $z$. 
Therefore, before start of the algorithm, the $len$ value of every node is at most $2k$. We now define the level of node $z$ as $\floor{\log len(z)}$ so that the total initial level of all the nodes is at most $2k (1+\log k)$. Suppose that a client $c$ is currently matched to $s$ by using a forward arc, and in a iteration gets rematched to $s'$ and $s$ gets rematched to $c'$ both again using forward arcs. At least one of $len(c)$ or $len(s)$ should have decreased by at least factor of $2$. And therefore the total level of $c$ and $s$ at least decreases by 1. In other words, on every rematch, the total level decreases by at least 1, which together with the bound on total initial level gives the number of such rematches to be at most $2k ( 1+\log k)$.
If at least one of $c$ or $s$ gets rematched by a reverse arc, its match does not change from then on. 
Thus, the number of these type of rematches are at most $2k$.
Thus, in total, the recourse of the algorithm is $O(k \log k)$.
\end{proof}


